Enabling Cost-Benefit Analysis of Data Sync Protocols

The problem of data synchronization arises in networked applications that require some measure of consistency. Indeed data synchronization approaches have demonstrated a significant potential for improving performance in various applications ranging from distributed ledgers to fog-enabled storage offloading for IoT. Although several protocols for data sets synchronization have been proposed over the years, there is currently no widespread utility implementing them, unlike the popular Rsync utility available for file synchronization. To that end, we describe a new middleware called GenSync that abstracts the subtleties of the state-of-the-art data synchronization protocols, allows users to choose protocols based on a comparative evaluation under realistic system conditions, and seamlessly integrate protocols in existing applications through a public API. We showcase GenSync through a case study, in which we integrate it into one of the world's largest wireless emulators and compare the performance of its included protocols.

==> content/abstract_v2.tex <==
Blockchain has recently emerged as a promising technology to improve
decentralization, interoperability, and transparency in IoT and
next-generation network applications. From accident forensics in
vehicular networks (VANET) of self-driving cars and information
poisoning prevention in mission-critical unmanned aerial vehicle
networks (UAANET) to IoT access management and security of federated
learning in fog computing, the blockchain's data integrity and
authenticity guarantees have been widely appreciated. However, the
questions of performance and scalability of traditional blockchains in
future 6G systems have received limited attention in the
literature. In this article, we focus on the performance of set
reconciliation; one of the main building blocks of recent block
propagation protocols. First, we discuss the advantages of set
reconciliation over traditional block propagation approaches and
identify the unique challenges to set reconciliation in the context of
next-generation networks and applications. Then, we introduce our
\gensync framework and use it to navigate the trade-off space
consisting of several popular set reconciliation algorithms. As a case
study, we integrate \gensync into \colosseum, a massive wireless
network emulator. Guided by the conclusions from this case study, we
envision a block propagation protocol architecture based on set
reconciliation to tackle the challenges of future mobile blockchains.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NOTES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Target call in IEEE Communications is
% https://www.comsoc.org/publications/magazines/ieee-communications-magazine/cfp/future-trends-fogedge-computing-and
% - Blockchains have emerged as a an appealing technology to implement
% _security and trust_ in fog/edge systems.

% The papers we're referring to:
% - IoT access management (Blockchain Meets IoT: An Architecture for
% Scalable Access Management in IoT)
% - IoT: Blockchain for Internet of Things: A Survey (IEEE Internet of
% Things Journal)
% - Federated learning in the fog (Decentralized Privacy Using Blockchain-Enabled
% Federated Learning in Fog Computing, IEEE Internet of Things Journal)
% - accident forensics in vehicular ad-hoc networks (Block4Forensic:
% An Integrated Lightweight Blockchain Framework for Forensics
% Applications of Connected Vehicles)
% - mission-critical unmanned aerial vehicle (Securing ICN-Based
% UAV Ad Hoc Networks with Blockchain)
% - Mneme: A Mobile Distributed Ledger (INFOCOM), a consensus protocol
% that reduces the storage needs when compared to traditional alternatives.

% The blockchain applications we can add:
% - Blockchain-Based Privacy-Aware Content Caching in Cognitive
% Internet of Vehicles
% - Fusion of Software Defined Networking,
% Edge Computing, and Blockchain Technology for Wireless Network
% Virtualization
% - When Internet of Things Meets Blockchain: Challenges in
% Distributed Consensus (2019), IEEE Network
% - A Bilayer Scalable Nakamoto Consensus Protocol for Blockchain
% Systems (2022), IEEE Network
% - Blockchain for Internet of Things: A Survey (Internet of Things
% Journal)
% - Groupchain: Towards a Scalable Public Blockchain in Fog Computing
% of IoT Services Computing
% - Analysis of the Communication Traffic for Blockchain Synchronization of IoT Devices

% Three-layer architecture:
% - Toward Blockchain-Powered Trusted
% Collaborative Services for Edge-Centric Networks; but different
% names for the layers
% - Toward ML/AI-Based Prediction of Mobile Service Usage in
% Next-Generation Networks (IEEE Network; Figure 1 when they present
% their simulation architecture)

% Where do we get the terms that we use throughout this paper:
% - 'Next-generation networks' (ManagingNext-GenerationNetworks
% forIntelligent Services and Applications; IEEE Network)
% - 'roadside unit' (Wireless Access Technologies for
% Vehicular Network Safety Applications)

% The terms we did not use but can consider using:
% - 6G-native blockchain design; for the blockchain of heterogeneous
% devices connected over heterogeneous networks.

% Somewhat related recent papers:
% - An In-Depth Review on Blockchain Simulators for IoT Environments
% (MDPI Article that cites CBlockSim; which is unrelated to this paper)

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> content/body_v2.tex <==
\section{Introduction}

\begin{figure*}[!t]
  \centering
  \includegraphics[width=1\linewidth]{drawings/distributed_ledger.pdf}
  \caption{Blockchain overlay on top of a next-generation network.}
  \label{fig:high_level}
\end{figure*}

\section{Fundamentals of Block Propagation in Blockchains}

\subsection{Modes of Operation}
Legacy, Compactblock (low bnadwidth, high bandwidth), Graphene

\subsection{Next-generation Challenges}
churn (Anas), bandwidth constraints, propagation to x\% of the network.

\section{Set Reconciliation}
The problem formulation.
\subsection{Existing Protocols}
Bloom filter, cuckoo filter, IBLT, CPI
\subsection{Trade-offs}

\section{Gossip-layer Design}
The proposed architecture

\section{Experimental Evaluation}

\subsection{\colosseum meets \gensync}
Describe the framework when embedded in Colosseum.

Show transfer-layer measurements.

Is there correlation between the transfer-layer latency-bandwidth
variations and attenuation on the physical layer?

\section{Related Work}
Graphene, Erlay...

\section{Set Reconciliation Beyond Blockchains}

\section{Conclusion}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

